Simple and Efficient Hard Label Black-box Adversarial Attacks in Low Query Budget Regimes

We focus on the problem of black-box adversarial attacks, where the aim is to generate adversarial examples for deep learning models solely based on information limited to output label~(hard label) to a queried data input. We propose a simple and efficient Bayesian Optimization~(BO) based approach for developing black-box adversarial attacks. Issues with BO's performance in high dimensions are avoided by searching for adversarial examples in a structured low-dimensional subspace. We demonstrate the efficacy of our proposed attack method by evaluating both $\ell_\infty$ and $\ell_2$ norm constrained untargeted and targeted hard label black-box attacks on three standard datasets - MNIST, CIFAR-10 and ImageNet. Our proposed approach consistently achieves 2x to 10x higher attack success rate while requiring 10x to 20x fewer queries compared to the current state-of-the-art black-box adversarial attacks.

==> experiments.tex <==
\section{Experiments}
Our experiments focus on the untargeted attack setting where, given an image correctly classified by the model, the goal is to produce an $\ell_p$-constrained perturbation such that applying this perturbation to the original image causes misclassification. We evaluate both $\ell_\infty$ and $\ell_2$ norm constrained hard label black-box attacks.
%We primarily consider performance of {Bayes-Attack} on ImageNet classifiers and compare its performance to other black-box attacks with respect to success rate over a given query budget. %, average query and median query. 
To compare performance, we randomly selected a subset of 1000 images, normalized to $[0,1]$, from the ImageNet validation set. In all experiments in this section, attacks are performed on this fixed set of images. We primarily compare performance of {Bayes-Attack} on ImageNet classifiers with that of other hard-label black-box attacks for small query budgets, and report success rates and average queries.
We also perform ablation studies on the ImageNet validation set by exploring different low dimension structured subspaces and examining different upsampling techniques.

% In this section, we present experiments and results.  We focus on the untargeted attack setting where the goal is to perturb the original image originally classified correctly by the classification model to cause misclassification. We consider the $\ell_\infty$ threat model on ImageNet \citep{imagenet} and MNIST \citep{mnist} and evaluate the performance in terms of 
% success rate over a given query budget, average query and median query. We perform ablation study on MNIST dataset by comparing different upsampling techniques. We also show the sensitivity of our method by varying the latent dimension $d'$ used to run Bayesian optimization on MNIST.

We define success rate as the ratio of the number of images successfully perturbed for a given query budget to the total number of input images. In all experiments, images that are already misclassified by the target network are excluded from the set; only images that are initially classified with the correct label are attacked. For each method of attack and each target network, we compute the success rate and average number of queries used to attack among images that were successfully perturbed. 



% We also show the white-box PGD results from \citet{madry2018towards}. {\color{red} talk about MNIST experiments here if they get finished}. 



% \begin{figure}[t]
% \centering
% \begin{subfigure}[b]{0.4\textwidth}
%   \includegraphics[width=\linewidth]{icml_legend.pdf}
% \end{subfigure}\\
% \begin{subfigure}[b]{0.3\textwidth}
%   \includegraphics[width=0.9\linewidth]{icml_bo_resnet.pdf}
%   \caption{{ResNet50}}
%   \label{fig:resnet} 
% \end{subfigure}
% \begin{subfigure}[b]{0.3\textwidth}
%   \includegraphics[width=0.9\linewidth]{icml_bo_inception.pdf}
%   \caption{{Inception-v3}}
%   \label{fig:inception}
% \end{subfigure}
% \begin{subfigure}[b]{0.3\textwidth}
%   \includegraphics[width=0.9\linewidth]{icml_bo_vgg.pdf}
%   \caption{{VGG16-bn}}
%   \label{fig:vgg}
% \end{subfigure}
% \caption{Performance comparison for $\ell_2$ untargeted attacks with $\epsilon=20.0$ on ImageNet classifiers. {Bayes-Attack} significantly outperforms all the other baselines.}
% \label{fig:imagenet_l2}
% \end{figure}

% \begin{table}[t]
% \centering
% \footnotesize
% \caption{Results for $\ell_2$ untargeted attacks on ImageNet classifiers with a query budget of $1000$}
% \begin{tabular}{c c  c c | c c | c c} 
%  \toprule
%  & &  \multicolumn{2}{c}{$\epsilon = 5.0$} &  \multicolumn{2}{c}{$\epsilon = 10.0$} & \multicolumn{2}{c}{$\epsilon = 20.0$}\\
% {{ \bf Classifier}} & {\bf Method} & {\bf Success} & {\bf Avg Queries} & {\bf Success} & {\bf Avg Queries} & {\bf Success} & {\bf Avg Queries}\\
%  \midrule
% \multirow{3}{*}{ {ResNet50}} 
%  &	{OPT attack}	& $	{2.16}	\% $ & $	{334.00}	 $ & $	                                    {4.71}	\% $ & $	{294.62}	 $ & $	                                    {9.03}	\% $ & $	{240.94}	 $ \\
% &	{Sign-OPT attack} & $	{4.07}	\% $ & $	{456.47}	 $ & $	                                    {6.62}	\% $ & $	{424.62}	 $ & $	                                    {12.98}	\% $ & $	{458.99}	 $ \\
% &	{Bayes attack}	& $	\mbf{20.10}	\% $ & $	\mbf{64.23}	 $ & $	                                \mbf{37.15}	\% $ & $	\mbf{64.13}	 $ & $	                                \mbf{66.67}	\% $ & $	\mbf{54.97}	 $ \\
% \midrule
% \multirow{3}{*}{{Inception-v3}}
% 	  &	{OPT attack} & $	{1.00}	\% $ & $	{277.75}	 $ & $	                                    {1.88}	\% $ & $ {221.47}		 $ & $	                                    {4.51}	\% $ & $	{247.67}	 $ \\
% &	{Sign-OPT attack} & $	{2.25}	\% $ & $	{648.50}	 $ & $	                                    {3.75}	\% $ & $ {611.77}		 $ & $	                                    {6.13}	\% $ & $	{557.71}	 $ \\
% &	{Bayes attack}	& $	\mbf{11.39}	\% $ & $	\mbf{109.65}	 $ & $	                            \mbf{22.65}	\% $ & $	\mbf{65.66}	 $ & $	                                \mbf{39.92}	\% $ & $	\mbf{68.86}	 $ \\
%   \midrule
%   \multirow{3}{*}{{VGG16-bn}}
%  &	{OPT attack}	 & $	{2.51}	\% $ & $	{204.47}	 $ & $	                                    {4.10}	\% $ & $	{176.32}	 $ & $	                                    {9.38}	\% $ & $	{229.77}	 $ \\ 
% &	{Sign-OPT attack} & $	{7.27}	\% $ & $	{552.33}	 $ & $	                                    {11.36}	\% $ & $	{476.57}	 $ & $	                                    {18.23}	\% $ & $	{417.46}	 $ \\
% &	{Bayes attack}	& $	\mbf{24.04}	\% $ & $	\mbf{69.84}	 $ & $	                                \mbf{43.46}	\% $ & $	\mbf{76.54}	 $ & $	                                \mbf{71.99}	\% $ & $	\mbf{48.95}	 $ \\
%  \bottomrule
%  \end{tabular}
%  \label{table:query_compare_l2}
%  \end{table}
 
 \begin{table*}[t]
 \centering
\footnotesize
\caption{Results for $\ell_2$ untargeted attacks on ImageNet classifiers with a query budget of $1000$}
\begin{tabular}{c l c c | c c | c c}
\toprule
\multicolumn{1}{l}{}          & \multicolumn{1}{l}{}  & \multicolumn{2}{c}{eps = 5.0}    & \multicolumn{2}{c}{eps = 10.0}  & \multicolumn{2}{c}{eps = 20.0}  \\

Classifier                    & Method                & success        & avg. query      & success        & avg. query     & success        & avg. query     \\
\midrule
\multirow{6}{*}{ResNet50}     & Boundary Attack       & 8.52           & 655.49          & 15.39          & 577.93         & 26.97          & 538.13         \\
                              & OPT attack            & 7.64           & 777.42          & 15.84          & 737.15         & 32.53          & 757.9          \\
                              & HSJA                  & 6.99           & 904.27          & 14.76          & 887.17         & 28.37          & 876.78         \\
                              & Sign-OPT              & 7.64           & 777.42          & 15.84          & 737.15         & 32.53          & 757.9          \\
                              & Sign-OPT-FFT          & 13.99          & 919.14          & 29.26          & 906.3          & 55.97          & 902.82         \\
                              & \textbf{Bayes attack} & \textbf{20.1}  & \textbf{64.23}  & \textbf{37.15} & \textbf{64.13} & \textbf{66.67} & \textbf{54.97} \\
\midrule
\multirow{6}{*}{Inception-v3} & Boundary Attack       & 0.38           & 998.67          & 6.88           & 588.24         & 14.52          & 531.06         \\
                              & OPT attack            & 3              & 820.79          & 6.88           & 673.71         & 16.27          & 722.75         \\
                              & HSJA                  & 1.63           & 878.54          & 5.51           & 882.48         & 12.89          & 887.8          \\
                              & Sign-OPT              & 7.13           & 839.57          & 14.26          & 831.76         & 22.78          & 837.91         \\
                              & Sign-OPT-FFT          & 7.13           & 929.32          & 15.39          & 924.64         & 34.79          & 917.27         \\
                              & \textbf{Bayes attack} & \textbf{11.39} & \textbf{109.65} & \textbf{22.65} & \textbf{65.66} & \textbf{39.92} & \textbf{68.86} \\
\midrule
\multirow{6}{*}{VGG16-bn}     & Boundary Attack       & 11.23          & 626.33          & 21.27          & 547.64         & 39.37          & 503.22         \\
                              & OPT attack            & 11.09          & 736.58          & 21.79          & 658.9          & 43.86          & 718.68         \\
                              & HSJA                  & 10.3           & 893.2           & 21.53          & 898.15         & 40.82          & 892.56         \\
                              & Sign-OPT              & 19.81          & 841.05          & 35.8           & 843.68         & 60.63          & 857.71         \\
                              & Sign-OPT-FFT          & 21.4           & 916.81          & 42.93          & 910.89         & 70.81          & 907.93         \\
                              & \textbf{Bayes attack} & \textbf{24.04} & \textbf{69.84}  & \textbf{43.46} & \textbf{76.54} & \textbf{71.99} & \textbf{48.95} \\
 \bottomrule
 \end{tabular}
 \label{table:query_compare_l2}
 \end{table*}
 
 
 
 
\subsection{Untargeted $\ell_2$ attack}
We compare the performance of the proposed method {Bayes-Attack} against Boundary attack\citep{brendel2017decision}, {OPT} attack\citep{cheng2018query}, HopSkipJump attack~(HSJA) \citep{Chen2019HopSkipJumpAttackAQ} and {Sign-OPT}\citep{signopt}, which is the current state of the art among hard-label black-box attacks within the $\ell_2$ threat model. We also compare our model to another version of Sign-OPT where we search the perturbation in a low dimensional subspace defined by FFT basis similar to the proposed method (Sign-OPT-FFT). 
On ImageNet, we attack the pretrained\footnote{Pretrained models available at \url{https://pytorch.org/docs/stable/torchvision/models}} models $-$ ResNet50 \citep{resnet}, Inception-v3 \citep{inception} and VGG16-bn \citep{vgg}.

We compare the performance across three different $\ell_2$ perturbation bounds, where we set $\epsilon$ to $5.0$, $10.0$ and $20.0$ respectively. We evaluate the performance of all the methods with a budget of up to 1000 queries. For the baseline methods, we use the implementations made available by the authors and use hyperparameters as suggested in their respective papers.
% provided by \citet{signopt} for {Sign-OPT}. Similarly for OPT attack, we use the publicly available implementation and hyperparameters reported in \citet{cheng2018query}.

%Similarly for {Parsimonious}, we use the implementation\footnote{\url{https://github.com/snu-mllab/parsimonious-blackbox-attack}} and hyperparameters given by \citet{parsimonious}.


% Figure \ref{fig:imagenet_l2} considers the the specific case of $\epsilon = 20.0$ in the above experiment, and exhibits the relationship between success rates and  number of queries used for each method.
%of the proposed method, {Bayes-Attack}, against the set of baseline methods in terms of success rate at different query budgets on $\ell_2$ untargeted attacks on ImageNet classifiers with perturbation bound $\epsilon = 20.0$.
 Table \ref{table:query_compare_l2} compares success rate and average query count of all methods, models, and $\epsilon$ thresholds for a query budget of $1000$. We can see that  {Bayes-Attack} consistently outperforms the other baseline methods across all classifiers and epsilons. %Bayes-Attack not only manages to achieve better attack success rates, but simultaneously reduces the average query count by up to a factor of ten. 
 As we can see from the table that searching for perturbation in low dimension Sign-OPT-FFT clearly improves over Sign-OPT but our proposed method Bayes-Attack achieves better success rates and hugely reduces the average query count by up to a factor of $10$ consistently over all the baseline methods. This huge reduction in query counts for finding adversarial perturbations can be contributed to efficiently searching for adversarial perturbations using Bayesian optimization.
 
%Even for query budgets $>200$, {Bayes-Attack} achieves better success rates than {Bandits-td} and {NES} on ResNet50 and VGG16-bn. Finally, we note that for higher query budgets $(>1000)$, both {Parsimonious} and {Bandits-td} method perform better than {Bayes-Attack}.


%To compare the success rate and average/median query, we select a point on the plots shown in Figure \ref{fig:imagenet}. Table \ref{table:query_compare} compares the performance of all the methods in terms of success rate, average and median query for a query budget of $200$. We can see that {Bayes-Attack} achieves higher success rate with $80\%$ less average queries as compared to the next best {Parsimonious} method.  Thus, we argue that although the Bayesian Optimization adversarial attack approach is to some extent a ``standard'' application of traditional Bayesian Optimization methods, the performance over the existing state of the art makes it a compelling approach particularly for the very low query setting. We also compare the average $\ell_2$ distortion of the generated adversarial perturbations in Appendix \ref{sec:l2_dist}.
% \begin{table}[h]
% \centering
% \caption{Results for $\ell_\infty$ untargeted attacks on ImageNet classifiers with a query budget of $1000$}
% \begin{tabular}{c c  c c } 
%  \toprule
% {{ \bf Classifier}} & {\bf Method} & {\bf Success} & {\bf Avg } \\
% & & {\bf Rate} &{\bf Queries}\\
%  \midrule
% \multirow{2}{*}{ {ResNet50}} 
 
% &	{Sign-OPT attack} & $  {3.05}	\% $ & $	{332.38}	 $ \\
% &	{Bayes attack}	& $	\mbf{67.48}	\% $ & $	\mbf{45.94}	$ \\
% \midrule
% \multirow{2}{*}{{Inception-v3}}
% &	{Sign-OPT attack} & $	{1.75}	\% $ & $	{549.00}	 $ \\
% &	{Bayes attack}	& $	\mbf{44.29}	\% $ & $	\mbf{72.31} $  \\
%   \midrule
%   \multirow{2}{*}{{VGG16-bn}}	            
% &	{Sign-OPT attack} & $	{5.81}	\% $ & $	{469.84}	 $  \\
% &	{Bayes attack}	& $	\mbf{78.47}	\% $ & $	\mbf{33.70}	 $  \\
%  \bottomrule
%  \end{tabular}
%  \label{table:query_compare_linf}
%  \end{table}





 





% \subsection{Experiments on MNIST}
% For MNIST, we use the pretrained network (used in \citet{carlini2017}) with $4$ convolutional layers, $2$ max-pooling layers and $2$ fully-connected layers which achieves $99.5\%$ accuracy on MNIST test set. We conduct $\ell_\infty$ untargeted adversarial attacks with perturbation bound $\epsilon = 0.2$ on a randomly sampled $1000$ images from the test set. 
% All the experiments performed on MNIST follow the same protocols.

% \subsubsection{Upsampling Methods}
% \label{sec:upsampling}
% The proposed method requires an upsampling technique for mapping the perturbation learnt in the latent dimension to the original input dimension.  In this section, we examine different linear and non-linear upsampling schemes and compare their performance on MNIST. The approaches we consider here can be divided into two broad groups: Encoder-Decoder based methods and Interpolation methods. For interpolation-based methods, we consider nearest-neighbor, bilinear and bicubic interpolation. 

% For encoder-decoder based approaches, we train a variational autoencoder \citep{kingma13,rezende14} by maximizing a variational lower bound on the log marginal likelihood. We also consider a simple autoencoder trained by minimizing the mean squared loss between the generated image and the original image. For both the approaches, we run the Bayesian optimization loop in latent space and use the pretrained decoder (or generator) for mapping the latent vector into image space. For these approaches, rather than searching for adversarial perturbation $\bm{\delta}$ in the latent space, we learn the adversarial image $\mbf{x} + \bm{\delta}$ directly using the Bayesian optimization. 

% Figure \ref{fig:upsampling} compares the performance of different upsampling methods. We can see that Nearest Neighbor ({\it NN}) interpolation and VAE-based decoder perform better than rest of the upsampling schemes. However, the {\it NN} interpolation 
% achieves similar performance to the VAE-based method but without the need of a large training dataset which is required for accurately training a VAE-based decoder.
 
%  \begin{figure}[t]
% \centering

% \begin{subfigure}[b]{0.49\textwidth}
%   \includegraphics[width=1\linewidth]{mnist_upsampling.pdf}
%   \caption{Performance comparison with different upsampling schemes.}
%   \label{fig:upsampling} 
% \end{subfigure}
% \begin{subfigure}[b]{0.49\textwidth}
%   \includegraphics[width=1\linewidth]{mnist_latent.pdf}
%   \caption{Performance comparison with different latent dimension.}
%   \label{fig:dimension}
% \end{subfigure}
% \caption{$\ell_\infty$ untargeted attacks on MNIST. {\it dim}: latent dimension used to run the Bayesian optimization, {\it NN}: Nearest neighbor interpolation, {\it BiC}: Bicubic interpolation, {\it BiL}: Bilinear interpolation, {\it AE}: autoencoder-based decoder, {\it VAE}: VAE-based generator (or decoder)}
% \label{fig:mnist}
% \end{figure}



% \subsubsection{Latent Dimension Sensitivity Analysis}
% We perform a sensitivity analysis on the latent dimension hyperparameter $d'$ used for running the Bayesian optimization. We vary the latent dimension over the range $d' \in \{9, 16, 64, 100, 256, 784\}$. Figure \ref{fig:dimension} shows the performance of nearest neighbor interpolation method for different latent dimension. We observe that lower latent dimensions achieve better success rates than the original input dimension $d'=784$ for MNIST. This could be because with increase in search dimension, Bayesian optimization needs more queries to find successful perturbation. 
% We also note that for the case of latent dimension $d'=9$, {Bayes-Attack} achieves lower success rates which could mean that it is hard to find adversarial perturbations in such low dimension. We show the convergence plots of {Bayes-Attack} on ImageNet and MNIST in Appendix \ref{sec:convergence}. 

%Therefore, for balancing both query counts and success rates we need to search for a optimal latent dimension.


% We can see that running {Bayes-Attack} in higher dimension is not always rewarding. This is because with increase in search dimension, Bayesian optimization takes more queries to find optimal solution. On the other hand, for much lower dimension $d'=9$ too, we observe that the success rates are low. 

% We perform ablation experiments described in supplementary material to compare the effectiveness of the configurations considered in our attack setup, i.e., selection of the structured low dimensional subspace and mapping techniques to generate adversarial perturbations in the original image space. We observe that the low frequency FFT basis vectors perform significantly better compared to random set of vectors generated from standard normal distribution in searching for adversarial perturbations. 

\subsection{Untargeted $\ell_\infty$ attack}
We also perform untargeted $\ell_\infty$ attacks with our model. We compare the performance of the proposed method {Bayes-Attack} against OPT \citep{cheng2018query} and {Sign-OPT} \citep{signopt}, which is the current state of the art among hard-label black-box attacks within the $\ell_\infty$ threat model.
We use the same query budgets, models, and reported metrics as in the previous subsection. Here, we set the $\ell_\infty$ perturbation bound $\epsilon$ to $0.05$. Table \ref{table:query_compare_linf} compares the performance of $\ell_\infty$ norm constrained attacks in terms of success rate and average query count. The proposed method Bayes-Attack consistently achieves significant performance improvements over the current methods.




 \begin{table*}[ht]
 \centering
\caption{Results for $\ell_\infty$ untargeted attacks on ImageNet classifiers with a query budget of $1000$}
\begin{tabular}{lcc| cc| cc}
\toprule
    & \multicolumn{2}{c}{ResNet50}                                 & \multicolumn{2}{c}{Inception-v3}        & \multicolumn{2}{c}{VGG16-bn}  \\
{\bf Method}               & {success} & {avg. query} & {success} & {avg. query} & {success} & {avg. query} \\
\midrule
OPT attack           & 5.73                        & 246.31                         & 2.87                        & 332.17                         & 7.53                        & 251.21                         \\
Sign-OPT             & 10.31                       & 660.37                         & 7.51                        & 706.3                          & 15.85                       & 666.87                         \\
\textbf{Bayes attack}    & \textbf{67.48}              & \textbf{45.94}                 & \textbf{44.29}              & \textbf{72.31}                 & \textbf{78.47}              & \textbf{33.7}   \\
\bottomrule
\end{tabular}
\label{table:query_compare_linf}
\end{table*}
